Understanding the illicit drug distribution in England: a data-centric approach to the County Lines Model

The County Lines Model (CLM) is a relatively new illicit drugs distribution method found in Great Britain. The CLM has brought modern slavery and public health issues, while challenging the law-enforcement capacity to act, as coordination between different local police forces is necessary. Our objective is to understand the territorial logic behind the line operators when establishing a connection between two places. We use three different spatial models (gravity, radiation and retail models), as each one of them understands flow from place i to j in a different way. Using public data from the Metropolitan Police of London, we train and cross-validate the models to understand which of the different physical and socio-demographic variables are considered when establishing a connection. We analyse hospital admissions by drugs, disposable household income, police presence and knife crime events, in addition to the population of a particular place and the distance and travel times between two different. Our results show that knife crime events and hospital admissions by misuse of drugs are the most important variables. We also find that London operators distribute to the territory known as the "South" of England, as negligible presence of them is observed outside of it.

==> lit_review.tex <==

\section{Literature review}
\label{sec:literature_review}

A literature review is done to document the work done until now in the scope of this work. 
%We centred the review in three different broad topics: the County Lines Model, The different quantitative approaches to tackle similar illicit drug distribution problems, and other works on illicit drugs around the world. 
Firstly, we describe the literature that has been published around the County Lines Model. Then, we review some of the quantitative methods that might be applied to the kind of problem we are facing, such as network science, econometrics and others. Finally, we present literature around the topic of illicit drugs distribution and consumption in the UK to understand the context of this work. At the end of this section we discuss the literature gap found and how from it we can tackle the research questions of this project. \\

%The review was done using \textit{scopus}, the Web of Science and the digital library of the University of Birmingham. We arrived to a set of 113 different peer-reviewed articles, from where 29 are cited in this review. The sets of questions that are intended to answer are: 
%\begin{itemize}
%    \item In which contexts are networks used for crime detection and analysis? How are these networks defined? Can they allow to implement the demand of different drugs? Have been criminal networks been analysed with a geographical element? Have they been analysed with a temporal element? Which mathematical/econometric/statistical techniques are used to analyse the given networks?
%    \item Has criminal networks analysis included exogenous elements in order to analyse their formation? Has the analysis included phenomena in the general population arisen from the network's formation?
%    \item Is there any quantitative work studying the appearance of the County Lines Model in the UK? Is there any quantitative work studying the heroin and/or cocaine import chain in the UK? \\
%\end{itemize} 

 In the case of the County Lines Model, only qualitative or official literature has been published. The Official literature includes documents and reports from different police agencies and the UK government. In particular, the NCA has published each year a statement regarding the views of the organisation about the County Lines Model \cite{NCA2018}. The document documents the findings from the NCA to understand the model and the different consequence it has had in the population.
 
 In 2019, the UK Government's Home Office commissioned an up-to-date report to be done around the illicit drugs problem in the UK. The report was published in eary 2020 \cite{Black2020_evidence, Black2020_summary} and reveals how the County Lines Model has evolved over the last decade. It also reports how the consumption of illicit drugs has changed in the population, stating that the UK faces an important challenge, as there currently are two peaks of consumers: one in their 20's and another in their 60's. Each one of those is of increasing worrisome, as the first one is the future workforce of the UK and the second represents an increasing pressure in the public services. 

Two different police organisations have publicly published information about the County Lines Model information they have. These are the Metropolitan Police of London \cite{Met2019, Met2020} and the West Midlands Police (Birmingham and metropolitan area) \cite{WestMidlands2020}. Only the Metropolitan Police has published quantitative data about their detection of lines in other police territories.

In January 2018, a debate was held in the House of Commons (UK's lower parliamentary chamber) to discuss the exploitation and harms done by the County Lines Model in London \cite{Commons2018}. Different Members of the Parliament asked what has been done until that point to tackle the CLM problems in London, particularly gang activity and exploitation.

Outside official documentation, academic literature about County Lines has mostly dedicated to report the child exploitation in different locations of England \cite{Andell2018, Robinson2019, Stone2018} and Scotland \cite{Gavin2018}. In all of them we find a description of the model. 
Ann anthropological study can be found in \cite{Ross2017}, where the authors interview different consumers and victims of the CLM in South England. \\

Given the nature of the data by the Metropolitan Police that is used for this study, we are interested in knowing the different methods involving networks and methods to analyse flows/transportation from one location to another. \\

Criminal networks analysis started to gain increasing popularity in criminology in the 90's \cite{Campana2016}. Originally defined as a specific and fixed form of organisation \cite{Podolny1998}, it slowly shifted to a more ``instrumental'' perspective \cite{Campana2016} where it is seen as a fluid and complex structure allowing to understand a criminal organisation \cite{Rostami2015}.

The more standard definition is to see a criminal network as a set of individuals (nodes) having a set of relations (links). In that sense, the criminal network can be defined by different kinds of participants, like offenders, consultants and \textit{ad hoc} workers, cooperating together with different kinds of relationships. These relationships, implemented as weights, can cover different types of cooperation between two nodes, like advisory, subordination or equality of ranks \cite{Campana2016}. However, different works have also studied more subjective attributes like trust between two individuals in the criminal network \cite{Bright2019}. This has come to the establishment of analysing Crime Networks as Social Networks. Most of the literature found for the literature review uses Social Networks Analysis as its framework and tool set to understand these criminal organisations \cite{Knoke2015, Campana2016, Bichler2017}. 

When characterising the edges and nodes, network analysis allows to know more about the structure of the criminal network, knowing its dimension and  hierarchies (small gang, organised gang, organised crime structure) \cite{Canter2004}, its efficiency and its robustness/security \cite{Morselli2007}.
To measure these three network's attributes, studies normally use the density of the network, and different centrality measures of the nodes \cite{Bichler2017, Berlusconi2017, Bright2019}. In particular, authors use the betweenness centrality as a measure for security/efficiency. Having a relatively small number of nodes with high betweenness centrality would mean a very efficient process but also a very centralised one, where taking down the strategic nodes would mean a disaster for the network. On the other hand, a more decentralised network would mean a higher robustness, as a larger number of nodes would be necessary to take down in order to make the network inoperable. We remind that, given a network with nodes $i=1,\ldots,N$, then the betweenness centrality of node $i$ is defined as
\begin{equation}
    \label{eq:betweenness}
    B_i=\sum_{j\neq k\neq i}\frac{\sigma_{i}(j, k)}{\sigma(j, k)},
\end{equation}
where $\sigma(j, k)$ is the total number of shortest paths going from node $j$ to node $k$, and $\sigma_i(j, k)$ is the number of shortest paths going from node $j$ to node $k$ \textit{passing through} $i$.
In that sense, betweenness centrality is a measure of how important is a given node to pass information within the network. 

It is here where we can also distinguish between two different broad topics in criminology literature: terrorist networks and criminal networks. \\

Terrorist networks became particularly relevant in academic literature after the 9/11 terrorists attacks \cite{Krebs2002,Lum2006}. Criminologists study the different individuals involved in these attacks and their different dynamics. The biggest difference between these two networks is the driving motif of the organisation to stay formed. While in a non-terrorist criminal network the driving force is economic and social profit, in terrorist networks the force gravitates more around ideology \cite{Krebs2002}. This elemental difference has important consequences in how the networks are structured. On the one hand, terrorist organisations care more about the robustness or security of their network. That is, if one or more elements fall down, the whole networks must not be exposed to fall down altogether. On the other hand, criminal organisations, by prioritising the economic profit of its network, their network would compromise robustness to increase their efficiency \cite{Morselli2007}. However, this last point is still highly debated in literature, as some authors still present arguments and cases where criminal networks opt for security over efficiency \cite{Berlusconi2017, Berlusconi2016}. \\

Criminology is the domain which has used a more diverse set of tools in order to analyse Crime Networks. In \cite{Dorsogna2015}, an important review has been done compiling the different approaches taken in the last two decades. We can split these approaches into three different categories: Agent based models (ABMs) \cite{Hegemann2011}, analytical models \cite{Short2010, Caminha2017} and network models \cite{Bright2019, Berlusconi2017}.  

Analytical models try to understand the formation and dissipation of criminal hot spots and other phenomena using PDEs \cite{Short2010}. ABMs and network models on the other hand have been developed to study the formation of criminal networks and the rehabilitation and recidivism of their members \cite{Berlusconi2017}.  

While analytical methods do not incorporate real data from the criminal networks or their locations, ABMs and networks have been including more data from recorded cases in the US, Mexico and different European countries \cite{Chandra2017, Chandra2015, Espinal2015}. \\

The SNA found in the literature tends to do not incorporate the temporal dimension. Networks are studied as snapshots in time, working with the nodes and links at a certain date. Only a handful of papers \cite{Bright2019, Berlusconi2017} have been found in which they incorporate different snapshots to the study. This kind of temporal study allows to better understand the key players and key relations that allow a criminal network to survive, while also understanding its fluidity and adaptation to internal changes \cite{Rostami2015}. \\

While most of the criminal networks studies focus in the organisation, formation and evolution, the literature involving the different illicit activities into place is smaller. Instead of focusing in networks as organisations of different sizes with individuals as nodes, these studies focus on geographical networks where nodes are more organised gangs in different geographical locations \cite{Berlusconi2017, Giommoni2017, Berlusconi2016, Dolliver2018}. The intention of the studies, located in an intersection between quantitative geography and economics, is to study the possible inflows and paths of illicit merchandise from one place to another tracking the price of the chosen merchandise. These can be MDMA in the US \cite{Chandra2017} or heroin in Europe \cite{Chandra2015}.  \\

A different but important method to note that has been used in the last decades is the study of the water sewage systems in different locations of the world. In particular, the European Monitoring Centre for Drugs and Drugs Addiction publishes every year the results obtained for different cities in Europe. The publication allows to monitor different drugs like cocaine, heroin and MDMA \cite{EMCDDA2020}. Normally, London appears in the top cities with cocaine and heroin consumption, although other British cities have appeared in the top rankings, such as Bristol \cite{EMCDDA2018}. \\

A notable element in most of the papers read for this literature review is the lack of an exogenous/prior context or data which would explain the criminal networks. In that sense, all of the criminal networks, social or geographical, are supposed already formed and static. Only one article \cite{Bright2019} was found in which the authors give a prior explanation about the context in which the analysed criminal social network was formed. However, this external information is only qualitative and does not have any data which can be used as input into the quantitative analysis, even though the necessity of it has been mentioned as a key element for analysing and predicting crime \cite{Hardyns2018}. \\

The literature found for illicit drug networks in the UK studies the inflow of drugs and the organisation of the criminal networks from an international perspective, always studying the UK parallel to Europe, the US \cite{Dolliver2018} or South Asia \cite{Ruggiero2007}. \\

In the case of the County Lines model, no quantitative analysis has been made. This is because of different elements: not enough data about gangs and the different routes used is publicly available; there is no data about the capacity and the volume of illicit drugs that these gangs are able to transport; there is no information about what is the share of sells in the illicit market attributed to the model. 

Given the lack of information, we cannot perform a Social Network Analysis, simply because we do not have any information about the elements of the organisation. 
In that sense, we cannot approach the problem in a similar way as those used for the inference of inflow paths by price analysis \cite{Berlusconi2017, Chandra2017, Chandra2015, Boivin2014}, where specific information about the organisations is omitted, only supposing that the gangs/cartels exist and have enough capacity to move merchandise from one place to another and consumers which would buy it at the objective location. The problem we have with this latter approach is that we could not suppose which are the capacities for other important exporters outside London.

The water sewage approach, although very interesting and conclusive, cannot be used in this framework given the specifications of the county lines model, tending to open local retailers in deprived and small towns, where the water sewage analysis has never been done. Indeed this particular analysis is only done in big cities in Europe, and does not have any data for more smaller and rural places in England. \\

The literature gap we have detected following this literature review is the lack of a quantitative analysis of the County Lines Model in England taking into account all the qualitative research done until now and the public data published by the Metropolitan Police of London.
%a temporal study taking into account more than 5 temporal points in which public data is used to infer capacity and possible paths, not only as emergent phenomena (prices), but also as inherent cause (deprivation). 
%The study case would be England, which could be divided in different topologies to increase or reduce the resolution of the study. 
%By incorporating the County Lines Model, proximity correlations would be erased, thus also showing a non-expected behaviour in a context where this kind of correlation would seem given. Having a quantitative model for England at such a resolution in crime networks would also a be a novel approach. 

A large number of network models can be adapted to our methodology. However, the work in \cite{Piovani2018} has proven to be the most adaptable, given that the analysis can incorporate different variables in a non-linear way, and by being derived from different constraints with respect to demand and spending power. The different models presented there and that are introduced in a more detailed form in Section \ref{sec:methods} has been used before for retail systems and for the London riots in 2012 \cite{Davies2013}, for human mobility studies \cite{Yang2014, Simini2012}, and more recently in exploring ancient trading routes in bronze-age Mesopotamia \cite{Barjamovic2019}, making them highly adaptable models.

%Different elements from the literature review done are going to be incorporated into the methodology used for this work. In a first place, the inference of inflow paths following the distribution of prices will be incorporated. However, given the lack of data for local prices in remote areas, we will have to adapt the methodology to other known variables, such as total numbers of seizures of drugs. Also, different qualitative arguments found in the literature about how deprivation levels are associated with a quicker and more resilient criminal network over time will be incorporated to our quantitative analysis. This would allow to incorporate an exogenous prior context as a quantitative variable into our model. 

%In \cite{Berlusconi2017}, the authors use a node similarity measure to argue the adaptation of the criminal network in case one of the nodes is expelled from it (by any relevant factor). The idea can be adapted to geographical locations, where a similarity can be found to assure that the county model survives with a diversification of supply routes. 

From the literature cited above, we can also outline the different hypotheses we work with throughout this work. By the different official and academic literature around county lines \cite{Black2020_summary, Coombes2018, Andell2018, Robinson2019, Stone2018}, we can suppose that \\

\textit{H1: county lines model does not take population and distance as a primordial element to establish a connection} \\

Thus making the traditional gravity model used here as the expected worse model to perform. On the other hand of the scale, given that the Retail Model allows to have as input different social and demographic models, we thus have as second hypothesis that: \\

\textit{H2: given the nature of the model, the Retail model will be the best performing of all.} \\

Also, given the literature around county lines, we can expect that from the different variables used in the Retail model (disposable income, police workforce, knife crime events, hospital admissions by misuse and hospital admissions by poisoning of drugs). \\

\textit{H3: the gross dispensable household income are an incentive for operators while the other four are costs for the operators.}

==> results.tex <==
\section{Results}
\label{sec:results}

\subsection{Model selection}
Results for the BIC and the S\o{}rensen-Dice index are found in Figure \ref{fig:BIC} and in Figure \ref{fig:Sorensen} respectively. 

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/BIC3.pdf}
        \caption{\label{fig:BIC}}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/Sorensen3.pdf}
        \caption{\label{fig:Sorensen}}
    \end{subfigure}
    \caption{\label{fig:indices}Results of BIC and the S\o{}rensen-Dice index for the 72 different models tested. Zone 0 corresponds to the Gravity model. Zone 1 corresponds to the Radiation model. Finally, zones 2 and 3 corresponds to the retail model with the Poissonian loss function and with the MSE loss function respectively. The annotated year corresponds to the data in which the model was trained on. Details of each model can be found in Appendix A.}
\end{figure}

When comparing the Retail model calibrated with a Gaussian loss function (zone 3 in Figure \ref{fig:indices}) with respect to the other models, we observe how the former performs worst in all of its forms for both the BIC and the $S$ index. We can thus proceed to discard these models.

Focusing in the models left, we note two different elements. First, still talking about the Retail model, but now with a Poissonian likelihood, we observe a trend where increasing the number of parameters $\alpha_n\neq 0$ decreases the performance of the model in both comparison measures. The best results obtained for the retail models are for two combinations: (1) $\alpha_n=0 \ \forall n$, and (2) $\alpha_3=-1.858\mathrm{e-}3\pm 4.792\mathrm{e-}4$ and $\alpha_n=0,$ for $n\neq 3$.

The parameter $\alpha_3$ corresponds to the police workforce \textit{per capita}, interpreted as a retail model where the police presence (\textit{per capita}) is a relevant factor for line operators to establish a connection between two places. The exponent in Eq. (\ref{eq:BLV_modified}) would take the form $\exp\{\alpha_3\log w_j^{(3)}-\beta c_{ij}\}$ in this case. 
The fact that $\alpha_3<0$ is interpreted as a negative correlation between the line operators and police presence. This by itself is of no surprise, as increasing police presence should in principle decrease the presence of crime. However, the result is interpreted as a nice reality check. 

On the other hand, the model corresponding to $\alpha_n=0$ has been mentioned in the literature \cite{Piovani2017} as a modified gravity model, as it only depends on the travel times from $i$ to $j$. In this case, the exponent in Eq. (\ref{eq:BLV_modified}) takes the form $\exp\{-\beta c_{ij}\}$. We will refer to it as the retail-gravity model from now on. \\

The second element to note is the discrepancy in the results of the Gravity models in Eq. (\ref{eq:gravity_modified}) for the BIC and S measurements. While for the $S$ index both gravity models (first two points from left to right) have high mean $S$ index, with the Gravity-Gaussian model having the third best score, we observe how they both perform poorly with the BIC, obtaining two of the three highest scores. 

Something similar happens with the Radiation-Gauss model, obtaining a high $S$ score but also a very high BIC value. On the other hand, the Radiation-Poisson model is the best performing model for both measurements. In Table \ref{tab:results_calibration} we present the results for the best three models found in our analysis: Radiation model and two forms of the Retail model, all of them calibrated with a Poissonian loss function. 

\hspace*{-2cm}
\begin{table}[h!]
    \centering
    \caption{\label{tab:results_calibration}Results for the best models calibrated.}
    \begin{tabular}{c|c|c|c|c|c}
         Ranking & Model & Loss function & Mean $S (S_{2019}, S_{2020})$ & BIC & Parameters \\
         \hline
        1 & Radiation & Poisson & 0.6377 & 4902 & \shortstack[l]{$\rho=3.678\pm 7.179\mathrm{e}-7$, \\$r=2.026\pm4.879\mathrm{e}-2$}  \\
        2 & Retail & Poisson & 0.6244 & 5078 & $\beta = 1.401\mathrm{e}-2\pm 8.471\mathrm{e}-5$  \\
        3 & Retail-Gravity & Poisson & 0.6236 & 5108 & \shortstack[l]{$\alpha_3=-1.858\mathrm{e}-3\pm 4.792\mathrm{e-}4$,\\ $\beta = 1.401\mathrm{e}-2\pm 8.477\mathrm{e}-5$} \\
    \end{tabular}
\end{table}

\subsection{Model analysis and geographic distribution}
Once we have obtained the best performing models, we proceed to compare and analyse the simulated distribution of modelled lines. In Figure \ref{fig:dispersion} we present the different models compared with the Metropolitan Police Data for 2019 and 2020. \\

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/dispersion_19.pdf}
        \caption{\label{fig:dispersion_19}}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/dispersion_20.pdf}
        \caption{\label{fig:dispersion_20}}
    \end{subfigure}
    \caption{\label{fig:dispersion}Data points and modelled lines ordered by police force for 2019 (a) and 2020 (b). Note: for both years, there were 0 lines detected in Durham. As the plot is in log scale, this data point was not included.}
\end{figure}

The three models tend to overestimate the detected connections to places with less than 100 lines, while underestimating them in police territories with more than 100 lines detected. 

While model 3 (Retail-police) in Table \ref{tab:results_calibration} has an extra factor included, in Figure \ref{fig:dispersion} we can observe how the introduction of $\alpha_3$ does not have any effect on modelling connections with respect to model 2 (Retail-gravity). Both models are overlapped and the difference between both is negligible. This is due to the order of magnitude of $\alpha_3\log w_j^{(3)}$ with respect to $\beta c_{ij}$. While the former element lies between [-9.113e-3, -1.663e-2], the second lies between [0.000, 0.455].
This encourage us to treat both of the Retail models as one. The negative correlation with police workforce, although an interesting element for our models, is marginal with respect to the impact of travel times $c_{ij}$ in the model. In what is left of the present work, we will then only focus in the Retail-Gravity model, as we can lower the number of free parameters to 1. \\

We are thus analysing two final models: the Radiation model and the Retail-Gravity model. Each one of them have different ways of understanding the dispersion of flow in a given space. On the one hand, the calibrated Radiation model sees the flow from London to another given police territory as a process of sorting opportunities presented on the way. After our calibration, opportunities here are seen as proportional to the population by the value of $\rho$ given in Table \ref{tab:results_calibration}. Thus, we are actually exploring how the population is distributed in England, if this particular distribution can have an insight about the observations by the Metropolitan Police of London.

On the other hand, the Retail-gravity model understands flow as a balance with respect to travel times using an exponential distribution. This means that flow from London to another police territory is given by how much time is spent commuting with respect to the other police territories. Thus, a closer place from London would be favoured with respect to a farther one. However, given that this consideration is given by an exponential distribution, we can expect a slow decrease of lines when increasing travel times (light tail distribution).  \\

\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_19.png}
        \caption{\label{fig:data_19}}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/rad_19.png}
        \caption{\label{fig:rad_19}}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/ret0_19.png}
        \caption{\label{fig:ret0_19}}
    \end{subfigure}
    
    \hfill
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/data_20.png}
        \caption{\label{fig:data_20}}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/rad_20.png}
        \caption{\label{fig:rad_20}}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/ret0_20.png}
        \caption{\label{fig:ret0_20}}
    \end{subfigure}
    \caption{\label{fig:models}Heatmaps for the Metropolitan Police data for 2019 (\ref{fig:data_19}) and 2020 (\ref{fig:data_20}), and the three different models tested: Radiation (\ref{fig:rad_19} and \ref{fig:rad_20}) and Retail-Gravity (\ref{fig:ret0_19} and \ref{fig:ret0_20}).}
\end{figure}

To further understand the different results shown in Table \ref{tab:results_calibration} and in Figure \ref{fig:dispersion}, we map the different  models and compare them with the Metropolitan Police data. This is shown in Figure \ref{fig:models}. While Figure \ref{fig:data_19} and \ref{fig:data_20} present the Metropolitan Police data for 2019 and 2020, the rest present the modelled spatial distribution of lines.
We also present the differences between the Metropolitan Police data and the models in Figure \ref{fig:diff}. Red zones correspond to territories overestimated by the model, while blue zones correspond to territories underestimated by the model. A similar map depicting the population in England in 2019 is shown in Figure \ref{fig:population_19}.\\

We start by analysing Figures \ref{fig:data_19} and \ref{fig:data_20} corresponding to the Metropolitan Police data. The first thing to notice is the decrease of detected lines in 2020 with respect to 2019. This effect can be given by mainly two factors taking into account the COVID-19 situation throughout 2020: the police had a smaller capacity to detect, or indeed the reduced mobility in the country reduced the number of connections. However, the decrease is not generalised and we can observe an increase in some police territories from 2019 to 2020, as in Hampshire (South of England) where we find the maximum number for 2020. 

A second element is important to note from the ground truth data. A very high share of the total lines (94.02\% for 2019 and 93.77\% for 2020) is concentrated in 16 out of the 37 police territories considered. This set of 16 police territories, in addition to London, is considered to be the ``South'' of England, a social region with no administrative recognition which encloses the most developed part of England and which opposes the ``North'' of England, where more industrial cities like Birmingham, Manchester and Liverpool are found (for a study using percolation theory please refer to \cite{Arcaute2016}).  \\


The ``North-South'' division is an element which none of the models captured. However, we can still see different ways of simulating the problem in Figures \ref{fig:rad_19}, \ref{fig:ret0_19}, \ref{fig:rad_20} and \ref{fig:ret0_20}. As discussed before, the Retail-Gravity model distributes the lines in what appears a concentric fashion with respect to London, leaning towards the centre of England. This can be seen more clearly in Figures \ref{fig:ret0_19_diff} and \ref{fig:ret0_20_diff}, where we observe an overestimation in the Midlands and an underestimation of the coastal territories of the ``South''.  Note how the far South west of England (Cornwall and Devon), which is farther away in travel times than the centre of England from London, is underrepresented. This fact accounts for an argument in which the operators in London would not have as primordial element for establishing connections the travel times to the different territories. This argument is supported by the opposite fact, where we observe an overestimation by the retail-gravity model in more connected places from London, like the West Midlands (Birmingham) and Warwickshire (south of Birmingham).

The radiation model understands the flow in a different fashion, as seen in Figures \ref{fig:rad_19} and \ref{fig:rad_20}. As for the Retail-Gravity model, the ring surrounding London is still catching an important number of lines. However, we can also observe a number of relatively large hotspots, particularly in West Yorkshire (North of England) and in West Mercia (border with Wales). While the former territory includes important cities and urban centres such as Leeds and Bradford, West Mercia is a diverse territory with dense suburban counties belonging to the Birmingham metropolitan area and more rural areas towards Wales, like Shropshire. In Figures \ref{fig:rad_19_diff} and \ref{fig:rad_20_diff} we observe also how the territories between West Yorkshire and London were filled with lines by the Radiation model. It is also important to note how the big metropolitan areas in England such as Birmingham and Manchester do not appear as hotspots in Figures \ref{fig:rad_19} and \ref{fig:rad_20}. Comparing the results of the Radiation model with respect to the distribution of the population in England (Figure \ref{fig:population_19}), we can ob serve how administrations like Cornwall and Devon or Avon and Somerset are closer to the Metropolitan Police data. This is in contrast to the results of the Retail-Gravity model. However, the distribution of population cannot explain the different maximums observed in 2019 (Norfolk) and 2020 (Hampshire). \\
  

Both models tend to distribute the number of lines in the centre of England, while avoiding the big cities. They also do not detect the territories where the maximum number of lines are detected, like Norfolk in 2019 and Hampshire in 2020. On one hand this is a sign of no overfitting from both models, but on the other hand makes very difficult for the models to detect future hotspots in the South of England.


\begin{figure}[ht]
    \centering    
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/rad_19_diff.png}
        \caption{\label{fig:rad_19_diff}}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/ret0_19_diff.png}
        \caption{\label{fig:ret0_19_diff}}
    \end{subfigure}
    \vfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/rad_20_diff.png}
        \caption{\label{fig:rad_20_diff}}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/ret0_20_diff.png}
        \caption{\label{fig:ret0_20_diff}}
    \end{subfigure}
        \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/population_19.png}
        \caption{\label{fig:population_19}}
    \end{subfigure}
    \caption{\label{fig:diff}Heatmaps showing the difference between the modelled distribution of lines with respect to the Metropolitan Police data for 2019 and 2020.}
\end{figure}
